RestainNet: a self-supervised digital re-stainer for stain normalization

Color inconsistency is an inevitable challenge in computational pathology, which generally happens because of stain intensity variations or sections scanned by different scanners. It harms the pathological image analysis methods, especially the learning-based models. A series of approaches have been proposed for stain normalization. However, most of them are lack flexibility in practice. In this paper, we formulated stain normalization as a digital re-staining process and proposed a self-supervised learning model, which is called RestainNet. Our network is regarded as a digital restainer which learns how to re-stain an unstained (grayscale) image. Two digital stains, Hematoxylin (H) and Eosin (E) were extracted from the original image by Beer-Lambert's Law. We proposed a staining loss to maintain the correctness of stain intensity during the restaining process. Thanks to the self-supervised nature, paired training samples are no longer necessary, which demonstrates great flexibility in practical usage. Our RestainNet outperforms existing approaches and achieves state-of-the-art performance with regard to color correctness and structure preservation. We further conducted experiments on the segmentation and classification tasks and the proposed RestainNet achieved outstanding performance compared with SOTA methods. The self-supervised design allows the network to learn any staining style with no extra effort.

==> 4.dataset.tex <==
%!Tex root=./tmi.tex

\section{Datasets}\label{sec4}
We evaluate our proposed PDBL in the following two datasets Kather Multiclass Dataset~\cite{kather} and LC25000 Dataset~\cite{LC25000}.
\subsection{Kather Multiclass Dataset}\label{kather_dataset}
Kather Multiclass Dataset is a multi-class colorectal dataset composed of H\&E stained histopathological tissue patches, which was published by J. N. Kather\footnotemark[2]. Kather Multiclass Dataset is composed of two subsets. Kather~\etal~\cite{kather} manually delineated tissue regions in $86$ colorectal~(CRC) tissue slides and they extracted $100,000$ H\&E histopathological tissue patches from these regions as Kather Multiclass Internal~(KMI) subset at $20\times$ magnification. They also extracted an additional independent Kather Multiclass External~(KME) subset include $7180$ H\&E stained histopathological patches. Histopathological images in Kather Multiclass Dataset are cropped to a square size of $224\times 224$ pixels from primeval whole slide images~(WSIs) at $20\times$ magnification.

As shown in Fig.~\ref{kather_fig}, each histopathological image belongs to one category of tissues and there are $9$ categories of tissues in Kather Multiclass Dataset such as adipose (ADI), background (BACK), debris (DEB), lymphocytes (LYM), mucus (MUC), smooth muscle (MUS), normal colon mucosa (NORM), cancer-associated stroma (STR), and colorectal adenocarcinoma epithelium (TUM).

\footnotetext[2]{\url{https://zenodo.org/record/1214456}}

\subsection{LC25000 Dataset}\label{lcdataset}
To advance computer-aided automated analysis of lung and colon carcinomas, \cite{LC25000} released a lung and colon histopathological image dataset (LC25000 Dataset)\footnotemark[3]. In LC25000 Dataset, histopathological images are cropped to a square size of $768\times 768$ pixels from H\&E stain WSIs of lung carcinoma and colon carcinoma. As shown in Fig.~\ref{fig:lc25000dataset}, LC25000 Dataset has $5$ categories such as benign lung tissues~(LN), lung adenocarcinomas~(LAC), lung squamous cell carcinomas~(LSCC), benign colonic tissues~(CN), and colon adenocarcinomas~(CAC). LC25000 Dataset is a balanced dataset that each class that has $5000$ histopathological images.

\footnotetext[3]{\url{https://github.com/tampapath/lung_colon_image_set}}


\begin{figure}[t]
    \setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}{ccccc}
        \includegraphics[width=.195\linewidth]{ADI.png}&
        \includegraphics[width=.195\linewidth]{BACK.png}&
        \includegraphics[width=.195\linewidth]{DEB.png}&
        \includegraphics[width=.195\linewidth]{LYM.png}&
        \includegraphics[width=.195\linewidth]{MUC.png}\\
        ADI & BACK & DEB & LYM & MUC \\
    \end{tabular}
    \begin{tabular}{cccc}
        \includegraphics[width=.195\linewidth]{MUS.png}&
        \includegraphics[width=.195\linewidth]{NORM.png}&
        \includegraphics[width=.195\linewidth]{STR.png}&
        \includegraphics[width=.195\linewidth]{TUM.png}\\
        MUS & NORM & STR & TUM\\
    \end{tabular}
    \caption{Kather Multiclass Dataset includes Adipose~(ADI), background~(BACK), debris~(DEB), lymphocytes~(LYM), mucus~(MUC), smooth muscle~(MUS), normal colon mucosa~(NORM), cancer-associated stroma~(STR), colorectal adenocarcinoma epithelium~(TUM).}
    \label{kather_fig}
\end{figure}

\begin{figure}[t]\centering
    \setlength{\tabcolsep}{1pt}
    \begin{tabular}{ccccc}
        \includegraphics[width=.195\linewidth]{lc_l_n.jpeg}&
        \includegraphics[width=.195\linewidth]{lc_l_ca.jpeg}&
        \includegraphics[width=.195\linewidth]{lc_l_scc.jpeg}&
        \includegraphics[width=.195\linewidth]{lc_c_n.jpeg}&
        \includegraphics[width=.195\linewidth]{lc_c_ca.jpeg}\\
        LN & LAC & LSCC & CN & CAC\\
    \end{tabular}
    \caption{LC25000 Dataset has 5 classes which includes benign lung tissues~(LN), lung adenocarcinomas~(LAC), lung squamous cell carcinomas~(LSCC), benign colonic tissues~(CN) and colon adenocarcinomas~(CAC)}
    \label{fig:lc25000dataset}
\end{figure}


\if 0
\subsection{Evaluation Metrics}
In this section, details of evaluation metrics are given. Accuracy and Macro-F1 score are utilized to evaluate the performance of the proposed PDBL.

Accuracy measures the proportion of correct classifications:
\begin{equation}
Accuracy = (TP+TN)/(P+N)
\end{equation}
where $TP$, $FP$, $TN$, and $FN$ represent true positive, false positive, true negative, and false negative, respectively. And $P$ and $T$ present the amount of positive group and negative group. F1 score contains information of precision score and recalls score which can be used to evaluate the performance of the multi-classification model more rigorously.

\begin{table*}[t]
	\centering
	\caption{Comparison of CNN backbones and PDBL on accuracy and macro-F1 score with complete training set (100\%).}
	\begin{tabular}{c|c|cc|cc|cc}
		\hline
		\multirow{2}{*}{Datasets}&\multirow{2}{*}{Models}
		&\multicolumn{2}{c|}{ResNet34}
		&\multicolumn{2}{c|}{EfficientNetb0}
		&\multicolumn{2}{c}{ShuffLeNetV2} \\ \cline{3-8}
		&&Accuracy&F1 score&Accuracy&F1 score&Accuracy&F1 score\\ \hline
		%%%%%%%%%%%%%%
		\multirow{2}{*}{Kather}
		&Baseline       &0.9503&0.9280&0.9504&0.9296&0.9546&0.9365\\ \cline{2-8}
		\multicolumn{1}{c|}{}
		&Baseline+PDBL  &$\mathbf{0.9547}$&$\mathbf{0.9334}$&$\mathbf{0.9582}$&$\mathbf{0.9392}$&$\mathbf{0.9611}$&$\mathbf{0.9444}$\\ \hline
		%%%%%%%%%%%%%%
		\multirow{2}{*}{LC25000}
		&Baseline       &0.9830&0.9830&0.9714&0.9714&0.9746&0.9746\\ \cline{2-8}
		\multicolumn{1}{c|}{}
		&Baseline+PDBL  &$\mathbf{0.9908}$&$\mathbf{0.9908}$&$\mathbf{0.9826}$&$\mathbf{0.9826}$&$\mathbf{0.9798}$&$\mathbf{0.9798}$\\ \hline
	\end{tabular}\label{tab:100}
\end{table*}

PRE is the precision score which can be calculated by:
\begin{equation}
PRE = TP/(TP+FP)
\end{equation}
and REC represents the recall score which can be calculated by:
\begin{equation}
REC = TP/(TP+FN).
\end{equation}

F1 score of the single class $n$ can be calculated by:
\begin{equation}
\text{F1}_n = 2\times (PRE\times REC)/(PRE+REC)
\end{equation}

In the multi-category classification tasks, Macro-F1 score is the average score of F1 scores for each class:
\begin{equation}
\text{F1} = \frac{1}{N}{\sum_{N}\text{F1}_k}
\end{equation}

In the rest of the paper, we use $\text{F1}$ to represent the macro-F1 score.
\fi

